Simulation-based Forecasting for Intraday Power Markets: Modelling Fundamental Drivers for Location, Shape and Scale of the Price Distribution

During the last years, European intraday power markets have gained importance for balancing forecast errors due to the rising volumes of intermittent renewable generation. However, compared to day-ahead markets, the drivers for the intraday price process are still sparsely researched. In this paper, we propose a modelling strategy for the location, shape and scale parameters of the return distribution in intraday markets, based on fundamental variables. We consider wind and solar forecasts and their intraday updates, outages, price information and a novel measure for the shape of the merit-order, derived from spot auction curves as explanatory variables. We validate our modelling by simulating price paths and compare the probabilistic forecasting performance of our model to benchmark models in a forecasting study for the German market. The approach yields significant improvements in the forecasting performance, especially in the tails of the distribution. At the same time, we are able to derive the contribution of the driving variables. We find that, apart from the first lag of the price changes, none of our fundamental variables have explanatory power for the expected value of the intraday returns. This implies weak-form market efficiency as renewable forecast changes and outage information seems to be priced in by the market. We find that the volatility is driven by the merit-order regime, the time to delivery and the closure of cross-border order books. The tail of the distribution is mainly influenced by past price differences and trading activity. Our approach is directly transferable to other continuous intraday markets in Europe.

==> TeX - Paper Submission Arxiv 1/00_acronyms.tex <==
%% Abkürzungen
\newacronym{SIDC}{SIDC}{Single IntraDay Coupling}
\newacronym{XBID}{XBID}{Cross Border Intraday}
\newacronym{RES}{RES}{Renewable Energy Sources}
\newacronym{GAM}{GAM}{Generalized Additive Models}
\newacronym{GAMLSS}{GAMLSS}{Generalized Additive Models for Location, Shape and Scale}
\newacronym{MAE}{MAE}{Mean Absolute Error}
\newacronym{RMSE}{RMSE}{Root Mean Squared Error}
\newacronym{CRPS}{CRPS}{Continuously Ranked Probability Score}
\newacronym{ES}{ES}{Energy Score}
\newacronym{DM}{DM}{Diebold-Mariano}
\newacronym{PB}{PB}{Pinball-Score}
\newacronym{WS}{WS}{Winkler-Score}
\newacronym{CR}{CR}{Coverage Ratio}
\newacronym{REMIT}{REMIT}{{Regulation on wholesale Energy Market Integrity and Transparency}}
\newacronym{LASSO}{LASSO}{{Least Absolute Shrinkage and Selection Operator}}
\newacronym{CDF}{CDF}{{Cumulative Distribution Function}}
\newacronym{PDF}{PDF}{{Probability Distribution Function}}
\newacronym{EEX}{EEX}{{European Energy Exchange}}
\newacronym{OTC}{OTC}{Over-The-Counter}
\newacronym{BIC}{BIC}{Bayesian Information Criterion}
\newacronym{MEH}{MEH}{Market Efficiency Hypothesis}
\newacronym{CET}{CET}{Central European Time}
\newacronym{CEST}{CEST}{Central European Summer Time}
\newacronym{TSO}{TSO}{Transmission System Operator}
\newacronym{AR}{AR}{Auto-Regressive}
\newacronym{ARX}{ARX}{Auto-Regressive with eXogenous input}
\newacronym{ARMA}{ARMA}{AutoRegressive Moving Average}
\newacronym{ARIMA}{ARIMA}{AutoRegressive Integrated Moving Average}
\newacronym{VWAP}{VWAP}{Volume-Weighted Average Price}
\newacronym{ACER}{ACER}{Agency for the Cooperation of Energy Regulators}
\newacronym{DA}{DA}{day-ahead}
\newacronym{ID}{ID}{intraday}
\newacronym{SDE}{SDE}{Stochastic Differential Equation}
\newacronym{PI}{PI}{Prediction Interval}
\newacronym{GARCH}{GARCH}{Generalized AutoRegressive Conditional Heteroscedasticity}

==> TeX - Paper Submission Arxiv 1/00_symbols.tex <==
%% Symbole

% Prices and price deltas
\newglossaryentry{symb:Pi}{name=$\pi^{d,s}_t$, description={Probability of at least one trade in the 5 minute interval $t$ on delivery day $d$ and hour $s$},sort=pi, type=symbolslist}
\newglossaryentry{symb:P}{name={$P$}, description={A price}, sort=P, type=symbolslist}
\newglossaryentry{symb:delta_P}{name={$\Delta P$}, description={First difference of $P$}, sort=P_delta, type=symbolslist}
\newglossaryentry{symb:P_d_s}{name={$P^{d,s}_t$}, description={The \gls{VWAP} at the 5-minute interval $t$}, sort=P_d_s, type=symbolslist}
\newglossaryentry{symb:delta_P_d_S}{name={$\Delta P$}, description={First difference of $P^{d,s}_t$}, sort=P_delta, type=symbolslist}

% time
\newglossaryentry{symb:d}{name=$d$, description={Delivery day},	sort=time_d, type=symbolslist}
\newglossaryentry{symb:s}{name=$s$,	description={Delivery hour in $s = \{0, ... ,S\}$ with $S=23$},	sort=time_s, type=symbolslist}
\newglossaryentry{symb:t}{name=$t$,	description={Simulation step in $t = \{1, ... ,T\}$},	sort=time_t, type=symbolslist}


% distributions
\newglossaryentry{symb:F}{name=$F$,	description={Some continuous distribution $F$},	sort=dist_F, type=symbolslist}
\newglossaryentry{symb:dirac}{name=$D_0$, description={The Dirac Distribution $D_0$}, sort=dist_dirac, type=symbolslist}
\newglossaryentry{symb:mu}{name=$\mu^F$, description={Location parameter of a distribtion $F$. Simplified as $\mu$},sort=dist_mu_F, type=symbolslist}
\newglossaryentry{symb:sigma}{name=$\sigma^F$, description={Scale parameter of a distribution $F$. Simplified as $\sigma$},	sort=dist_sigma, type=symbolslist}
\newglossaryentry{symb:nu}{name=$\nu^F$, description={First shape parameter of a distribtion $F$. Simplified as $\nu$},	sort=dist_nu, type=symbolslist}
\newglossaryentry{symb:tau}{name=$\tau^F$, description={Second shape parameter of a distribtion $F$. Simplified as $\tau$}, sort=dist_tau, type=symbolslist}
\newglossaryentry{symb:theta}{name=$\boldsymbol{\theta}^F$,	description={Parameter vector of a distribtion $F$},sort=dist_theta, type=symbolslist}

% variables (wind, solar etc)
\newglossaryentry{symb:MO}{name=$\textit{MO}^{d,s}_{q}$,	description={Slope of the merit order for $d,s$ for the price level at $t$ and $\pm q$ MW.},sort=var_mo, type=symbolslist}
\newglossaryentry{symb:W}{name=$\hat{W}^{d,s}_{t}$,	description={Wind production forecast for $d,s$ issued at $t$.},sort=var_w, type=symbolslist}
\newglossaryentry{symb:L}{name=$\hat{L}^{d,s}_{t}$,	description={Load forecast for $d,s$ issued at $t$.},sort=var_l, type=symbolslist}
\newglossaryentry{symb:S}{name=$\hat{S}^{d,s}_{t}$,	description={Solar production forecast for $d,s$ issued at $t$.},sort=var_s, type=symbolslist}


==> TeX - Paper Submission Arxiv 1/coefficients_table_mu_review.tex <==

\begin{tabular}{l>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}}
\toprule
  & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23\\
\midrule
$\alpha_{t-1}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F64E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E77A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EF6500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E57E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F55200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}}\\
$\alpha_{t-2}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F64E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\mid \Delta P_{t-1} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\mid \Delta P_{t-2} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F64E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\mid \Delta P_{t-3} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\mid \Delta P_{t-4} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\mid \Delta P_{t-5} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}}\\
$\mid \Delta P_{t-6} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\sum_{i=7}^{i=12} \mid \Delta P_{t-i} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\Delta P_{t-1}$ & \multicolumn{1}{r}{\cellcolor[HTML]{D99400}{-0.088}} & \multicolumn{1}{r}{\cellcolor[HTML]{DF8A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{DF8A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{D99400}{-0.084}} & \multicolumn{1}{r}{\cellcolor[HTML]{E48100}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{D1A000}{-0.071}} & \multicolumn{1}{r}{\cellcolor[HTML]{EB7000}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{CFA200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{B5C000}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.080}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.088}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.115}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.114}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.047}} & \multicolumn{1}{r}{\cellcolor[HTML]{49F700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{1FFD00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{61F100}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.071}} & \multicolumn{1}{r}{\cellcolor[HTML]{61F100}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{1FFD00}{0.045}} & \multicolumn{1}{r}{\cellcolor[HTML]{56F400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{CEA400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C6AE00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{D99400}{0.000}}\\
$\Delta P_{t-2}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F55200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F93E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74600}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F93E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F55200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.000}}\\
$\Delta P_{t-3}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{ED6A00}{0.034}} & \multicolumn{1}{r}{\cellcolor[HTML]{EA7200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$MO_{1000}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$MO_{2000}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F93E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F06200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$MO_{4000}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.036}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.028}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$L_{DA}$ & \multicolumn{1}{r}{\cellcolor[HTML]{DE8C00}{0.001}} & \multicolumn{1}{r}{\cellcolor[HTML]{ED6A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E87700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F25C00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{CFA200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F06200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C6AE00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F35800}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EF6500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F25C00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{CCA600}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F35800}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F64E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E57E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F93E00}{0.000}}\\
$O_{DA}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F45500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{DF8A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\Delta O$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\Delta O_{planned}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\Delta O_{unplanned}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\mid P_{Spot} - P_{t-1} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$SIDC$ & \multicolumn{1}{r}{\cellcolor[HTML]{E97500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E97500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EF6500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{DB9000}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C1B300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$S_{DA}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\Delta S^-$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\Delta S^+$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F35800}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\sigma S$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
TTD & \multicolumn{1}{r}{\cellcolor[HTML]{F06200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{ADC700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E57E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{DA9200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{8BDF00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EB7000}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C5B000}{0.054}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}}\\
MON(d) & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
SAT(d) & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
SUN(d) & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F25C00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$W_{DA}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74600}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F25C00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\Delta W^-$ & \multicolumn{1}{r}{\cellcolor[HTML]{EB7000}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F64E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.000}}\\
$\Delta W^+$ & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\sigma W$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.005}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
\bottomrule
\end{tabular}


==> TeX - Paper Submission Arxiv 1/coefficients_table_nu_review.tex <==

\begin{tabular}{l>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}}
\toprule
  & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23\\
\midrule
Intercept & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.003}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.034}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.011}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.033}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.008}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.026}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.025}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.005}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.010}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.006}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.001}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.035}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.015}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.017}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.044}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.042}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.006}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.017}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.032}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.025}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.022}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.065}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.002}}\\
$\alpha_{t-1}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\alpha_{t-2}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\mid \Delta P_{t-1} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\mid \Delta P_{t-2} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\mid \Delta P_{t-3} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\mid \Delta P_{t-4} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\mid \Delta P_{t-5} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\mid \Delta P_{t-6} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\sum_{i=7}^{i=12} \mid \Delta P_{t-i} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\Delta P_{t-1}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74600}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\Delta P_{t-2}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\Delta P_{t-3}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$MO_{1000}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$MO_{2000}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$MO_{4000}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$L_{DA}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74600}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$O_{DA}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\Delta O$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\Delta O_{planned}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\Delta O_{unplanned}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\mid P_{Spot} - P_{t-1} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$SIDC$ & \multicolumn{1}{r}{\cellcolor[HTML]{F45500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$S_{DA}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\Delta S^-$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\Delta S^+$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\sigma S$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
TTD & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{ED6A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
MON(d) & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
SAT(d) & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
SUN(d) & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$W_{DA}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\Delta W^-$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\Delta W^+$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\sigma W$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
\bottomrule
\end{tabular}


==> TeX - Paper Submission Arxiv 1/coefficients_table_sigma_review.tex <==

\begin{tabular}{l>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}}
\toprule
  & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23\\
\midrule
Intercept & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.277}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.302}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.464}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.700}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.551}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.206}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.178}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.490}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.426}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.060}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.044}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.551}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.876}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.700}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.813}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.918}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-1.045}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.724}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.799}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.730}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.742}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.727}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.654}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.347}}\\
$\alpha_{t-1}$ & \multicolumn{1}{r}{\cellcolor[HTML]{F93E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74600}{-0.052}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F15F00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EB7000}{-0.015}} & \multicolumn{1}{r}{\cellcolor[HTML]{EF6500}{-0.167}} & \multicolumn{1}{r}{\cellcolor[HTML]{EB7000}{-0.216}} & \multicolumn{1}{r}{\cellcolor[HTML]{F25C00}{-0.094}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F06200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EF6500}{0.000}}\\
$\alpha_{t-2}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\mid \Delta P_{t-1} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F45500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F55200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EC6D00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E87700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F55200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.295}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74600}{0.174}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F93E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EC6D00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EE6700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74600}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F25C00}{0.000}}\\
$\mid \Delta P_{t-2} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EF6500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74600}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F93E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F35800}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F45500}{0.000}}\\
$\mid \Delta P_{t-3} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F35800}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F93E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F93E00}{0.000}}\\
$\mid \Delta P_{t-4} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F64E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}}\\
$\mid \Delta P_{t-5} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}}\\
$\mid \Delta P_{t-6} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F93E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F93E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}}\\
$\sum_{i=7}^{i=12} \mid \Delta P_{t-i} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74600}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74A00}{0.000}}\\
$\Delta P_{t-1}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\Delta P_{t-2}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\Delta P_{t-3}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$MO_{1000}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{9DD300}{0.177}} & \multicolumn{1}{r}{\cellcolor[HTML]{F15F00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{ADC700}{0.267}} & \multicolumn{1}{r}{\cellcolor[HTML]{D29E00}{0.047}} & \multicolumn{1}{r}{\cellcolor[HTML]{E08700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EF6500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{D59A00}{0.101}} & \multicolumn{1}{r}{\cellcolor[HTML]{96D800}{0.319}} & \multicolumn{1}{r}{\cellcolor[HTML]{D99400}{0.198}} & \multicolumn{1}{r}{\cellcolor[HTML]{D69800}{0.038}} & \multicolumn{1}{r}{\cellcolor[HTML]{CBA800}{0.131}} & \multicolumn{1}{r}{\cellcolor[HTML]{D39C00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C6AE00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{DC8E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{B9BC00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C6AE00}{0.049}} & \multicolumn{1}{r}{\cellcolor[HTML]{D59A00}{0.138}} & \multicolumn{1}{r}{\cellcolor[HTML]{A0D100}{0.228}} & \multicolumn{1}{r}{\cellcolor[HTML]{DB9000}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F35800}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F25C00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C0B500}{0.150}}\\
$MO_{2000}$ & \multicolumn{1}{r}{\cellcolor[HTML]{BEB700}{0.285}} & \multicolumn{1}{r}{\cellcolor[HTML]{96D800}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{90DB00}{0.399}} & \multicolumn{1}{r}{\cellcolor[HTML]{DB9000}{0.024}} & \multicolumn{1}{r}{\cellcolor[HTML]{BCB900}{0.358}} & \multicolumn{1}{r}{\cellcolor[HTML]{E08700}{0.451}} & \multicolumn{1}{r}{\cellcolor[HTML]{ED6A00}{0.060}} & \multicolumn{1}{r}{\cellcolor[HTML]{73EA00}{0.378}} & \multicolumn{1}{r}{\cellcolor[HTML]{A9CA00}{0.244}} & \multicolumn{1}{r}{\cellcolor[HTML]{C1B300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{CBA800}{0.146}} & \multicolumn{1}{r}{\cellcolor[HTML]{DE8C00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{D29E00}{0.228}} & \multicolumn{1}{r}{\cellcolor[HTML]{E28300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F35800}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EE6700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E97500}{0.015}} & \multicolumn{1}{r}{\cellcolor[HTML]{C3B200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{BEB700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{61F100}{0.567}} & \multicolumn{1}{r}{\cellcolor[HTML]{B3C200}{0.249}} & \multicolumn{1}{r}{\cellcolor[HTML]{D99400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F55200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EE6700}{0.000}}\\
$MO_{4000}$ & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.239}} & \multicolumn{1}{r}{\cellcolor[HTML]{A4CE00}{0.471}} & \multicolumn{1}{r}{\cellcolor[HTML]{1FFD00}{0.459}} & \multicolumn{1}{r}{\cellcolor[HTML]{42F900}{0.680}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.352}} & \multicolumn{1}{r}{\cellcolor[HTML]{6FEC00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{49F700}{0.222}} & \multicolumn{1}{r}{\cellcolor[HTML]{B1C400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{7AE700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{66EF00}{0.252}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.213}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.170}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.264}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.405}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.420}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.572}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.705}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.831}} & \multicolumn{1}{r}{\cellcolor[HTML]{B7BE00}{0.454}} & \multicolumn{1}{r}{\cellcolor[HTML]{9DD300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{56F400}{0.336}} & \multicolumn{1}{r}{\cellcolor[HTML]{1FFD00}{0.355}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.315}} & \multicolumn{1}{r}{\cellcolor[HTML]{56F400}{0.183}}\\
$L_{DA}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$O_{DA}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\Delta O$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\Delta O_{planned}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\Delta O_{unplanned}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\mid P_{Spot} - P_{t-1} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F93E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}}\\
$SIDC$ & \multicolumn{1}{r}{\cellcolor[HTML]{DF8A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C1B300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{CEA400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C0B500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{D59A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{CEA400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C5B000}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C0B500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C3B200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C1B300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C9AA00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C6AE00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{D39C00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E08700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{D79600}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{DF8A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{DF8A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C9AA00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C6AE00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{BCB900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C5B000}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C9AA00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C0B500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C0B500}{0.000}}\\
$S_{DA}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\Delta S^-$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\Delta S^+$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\sigma S$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
TTD & \multicolumn{1}{r}{\cellcolor[HTML]{61F100}{0.226}} & \multicolumn{1}{r}{\cellcolor[HTML]{A9CA00}{0.122}} & \multicolumn{1}{r}{\cellcolor[HTML]{A9CA00}{0.172}} & \multicolumn{1}{r}{\cellcolor[HTML]{BEB700}{0.273}} & \multicolumn{1}{r}{\cellcolor[HTML]{AFC500}{0.265}} & \multicolumn{1}{r}{\cellcolor[HTML]{AFC500}{0.370}} & \multicolumn{1}{r}{\cellcolor[HTML]{7EE500}{0.410}} & \multicolumn{1}{r}{\cellcolor[HTML]{42F900}{0.425}} & \multicolumn{1}{r}{\cellcolor[HTML]{7EE500}{0.339}} & \multicolumn{1}{r}{\cellcolor[HTML]{AFC500}{0.309}} & \multicolumn{1}{r}{\cellcolor[HTML]{ABC900}{0.188}} & \multicolumn{1}{r}{\cellcolor[HTML]{7EE500}{0.294}} & \multicolumn{1}{r}{\cellcolor[HTML]{73EA00}{0.295}} & \multicolumn{1}{r}{\cellcolor[HTML]{A4CE00}{0.201}} & \multicolumn{1}{r}{\cellcolor[HTML]{A9CA00}{0.266}} & \multicolumn{1}{r}{\cellcolor[HTML]{A7CC00}{0.296}} & \multicolumn{1}{r}{\cellcolor[HTML]{A7CC00}{0.398}} & \multicolumn{1}{r}{\cellcolor[HTML]{7AE700}{0.301}} & \multicolumn{1}{r}{\cellcolor[HTML]{5CF200}{0.385}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.334}} & \multicolumn{1}{r}{\cellcolor[HTML]{8BDF00}{0.367}} & \multicolumn{1}{r}{\cellcolor[HTML]{66EF00}{0.339}} & \multicolumn{1}{r}{\cellcolor[HTML]{73EA00}{0.447}} & \multicolumn{1}{r}{\cellcolor[HTML]{39FA00}{0.332}}\\
MON(d) & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
SAT(d) & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
SUN(d) & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$W_{DA}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\Delta W^-$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\Delta W^+$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\sigma W$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
\bottomrule
\end{tabular}


==> TeX - Paper Submission Arxiv 1/coefficients_table_tau_review.tex <==

\begin{tabular}{l>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}>{\raggedright\arraybackslash}p{1.25cm}}
\toprule
  & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23\\
\midrule
Intercept & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.100}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.147}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.098}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.029}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.154}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.256}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.425}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.014}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.004}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.079}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.103}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.051}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.218}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.232}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.328}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.573}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.409}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{-0.014}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.072}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.111}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.101}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.044}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.013}} & \multicolumn{1}{r}{\cellcolor[HTML]{00FF00}{0.009}}\\
$\alpha_{t-1}$ & \multicolumn{1}{r}{\cellcolor[HTML]{A7CC00}{-0.186}} & \multicolumn{1}{r}{\cellcolor[HTML]{BCB900}{-0.064}} & \multicolumn{1}{r}{\cellcolor[HTML]{C5B000}{-0.086}} & \multicolumn{1}{r}{\cellcolor[HTML]{C3B200}{-0.095}} & \multicolumn{1}{r}{\cellcolor[HTML]{BEB700}{-0.074}} & \multicolumn{1}{r}{\cellcolor[HTML]{61F100}{-0.086}} & \multicolumn{1}{r}{\cellcolor[HTML]{B9BC00}{-0.120}} & \multicolumn{1}{r}{\cellcolor[HTML]{B5C000}{-0.080}} & \multicolumn{1}{r}{\cellcolor[HTML]{A9CA00}{-0.063}} & \multicolumn{1}{r}{\cellcolor[HTML]{E28300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C0B500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E28300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EB7000}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{D29E00}{-0.058}} & \multicolumn{1}{r}{\cellcolor[HTML]{C9AA00}{-0.054}} & \multicolumn{1}{r}{\cellcolor[HTML]{CFA200}{-0.075}} & \multicolumn{1}{r}{\cellcolor[HTML]{B5C000}{-0.141}} & \multicolumn{1}{r}{\cellcolor[HTML]{C9AA00}{-0.083}} & \multicolumn{1}{r}{\cellcolor[HTML]{B5C000}{-0.092}} & \multicolumn{1}{r}{\cellcolor[HTML]{CFA200}{-0.092}} & \multicolumn{1}{r}{\cellcolor[HTML]{9DD300}{-0.098}} & \multicolumn{1}{r}{\cellcolor[HTML]{B3C200}{-0.122}} & \multicolumn{1}{r}{\cellcolor[HTML]{B7BE00}{-0.119}} & \multicolumn{1}{r}{\cellcolor[HTML]{ABC900}{-0.128}}\\
$\alpha_{t-2}$ & \multicolumn{1}{r}{\cellcolor[HTML]{E18500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F25C00}{-0.032}} & \multicolumn{1}{r}{\cellcolor[HTML]{E67C00}{-0.039}} & \multicolumn{1}{r}{\cellcolor[HTML]{F25C00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E57E00}{-0.047}} & \multicolumn{1}{r}{\cellcolor[HTML]{DE8C00}{-0.037}} & \multicolumn{1}{r}{\cellcolor[HTML]{E18500}{-0.040}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74A00}{-0.040}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E97500}{-0.050}} & \multicolumn{1}{r}{\cellcolor[HTML]{EE6700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{-0.046}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F15F00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EE6700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EE6700}{-0.043}} & \multicolumn{1}{r}{\cellcolor[HTML]{F25C00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{-0.029}} & \multicolumn{1}{r}{\cellcolor[HTML]{EE6700}{-0.023}} & \multicolumn{1}{r}{\cellcolor[HTML]{F15F00}{-0.036}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{-0.003}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EE6700}{0.000}}\\
$\mid \Delta P_{t-1} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{CFA200}{0.227}} & \multicolumn{1}{r}{\cellcolor[HTML]{EC6D00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{AFC500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{ED6A00}{0.037}} & \multicolumn{1}{r}{\cellcolor[HTML]{BABB00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{9DD300}{0.208}} & \multicolumn{1}{r}{\cellcolor[HTML]{88E000}{0.215}} & \multicolumn{1}{r}{\cellcolor[HTML]{ADC700}{0.049}} & \multicolumn{1}{r}{\cellcolor[HTML]{C1B300}{0.057}} & \multicolumn{1}{r}{\cellcolor[HTML]{E57E00}{0.052}} & \multicolumn{1}{r}{\cellcolor[HTML]{EF6500}{0.034}} & \multicolumn{1}{r}{\cellcolor[HTML]{F93E00}{0.097}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E48100}{0.019}} & \multicolumn{1}{r}{\cellcolor[HTML]{DC8E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{D99400}{0.052}} & \multicolumn{1}{r}{\cellcolor[HTML]{C6AE00}{0.215}} & \multicolumn{1}{r}{\cellcolor[HTML]{DE8C00}{0.027}} & \multicolumn{1}{r}{\cellcolor[HTML]{A4CE00}{0.184}} & \multicolumn{1}{r}{\cellcolor[HTML]{EB7000}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E28300}{0.076}} & \multicolumn{1}{r}{\cellcolor[HTML]{C3B200}{0.217}} & \multicolumn{1}{r}{\cellcolor[HTML]{E67C00}{0.107}} & \multicolumn{1}{r}{\cellcolor[HTML]{ABC900}{0.127}}\\
$\mid \Delta P_{t-2} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{E18500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{BABB00}{0.099}} & \multicolumn{1}{r}{\cellcolor[HTML]{7AE700}{0.131}} & \multicolumn{1}{r}{\cellcolor[HTML]{D79600}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{CBA800}{0.103}} & \multicolumn{1}{r}{\cellcolor[HTML]{90DB00}{0.077}} & \multicolumn{1}{r}{\cellcolor[HTML]{B3C200}{0.088}} & \multicolumn{1}{r}{\cellcolor[HTML]{81E400}{0.128}} & \multicolumn{1}{r}{\cellcolor[HTML]{B1C400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{CEA400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E28300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.120}} & \multicolumn{1}{r}{\cellcolor[HTML]{ED6A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E87700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E67C00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{D79600}{0.048}} & \multicolumn{1}{r}{\cellcolor[HTML]{A2D000}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{D69800}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{CFA200}{0.051}} & \multicolumn{1}{r}{\cellcolor[HTML]{DC8E00}{0.033}} & \multicolumn{1}{r}{\cellcolor[HTML]{D69800}{0.122}} & \multicolumn{1}{r}{\cellcolor[HTML]{F06200}{0.058}} & \multicolumn{1}{r}{\cellcolor[HTML]{F55200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{A2D000}{0.104}}\\
$\mid \Delta P_{t-3} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{E67C00}{0.020}} & \multicolumn{1}{r}{\cellcolor[HTML]{A9CA00}{0.073}} & \multicolumn{1}{r}{\cellcolor[HTML]{A0D100}{0.060}} & \multicolumn{1}{r}{\cellcolor[HTML]{F06200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{D39C00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{A7CC00}{0.041}} & \multicolumn{1}{r}{\cellcolor[HTML]{D69800}{0.018}} & \multicolumn{1}{r}{\cellcolor[HTML]{93DA00}{0.007}} & \multicolumn{1}{r}{\cellcolor[HTML]{A9CA00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{DE8C00}{0.029}} & \multicolumn{1}{r}{\cellcolor[HTML]{E87700}{0.004}} & \multicolumn{1}{r}{\cellcolor[HTML]{F64E00}{0.025}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E97500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EC6D00}{0.053}} & \multicolumn{1}{r}{\cellcolor[HTML]{F35800}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C5B000}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C5B000}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{CFA200}{0.036}} & \multicolumn{1}{r}{\cellcolor[HTML]{EE6700}{0.052}} & \multicolumn{1}{r}{\cellcolor[HTML]{E08700}{0.038}} & \multicolumn{1}{r}{\cellcolor[HTML]{D29E00}{0.029}} & \multicolumn{1}{r}{\cellcolor[HTML]{ED6A00}{0.045}}\\
$\mid \Delta P_{t-4} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{D99400}{0.058}} & \multicolumn{1}{r}{\cellcolor[HTML]{BEB700}{0.051}} & \multicolumn{1}{r}{\cellcolor[HTML]{A9CA00}{0.013}} & \multicolumn{1}{r}{\cellcolor[HTML]{D1A000}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{7AE700}{0.088}} & \multicolumn{1}{r}{\cellcolor[HTML]{C3B200}{0.108}} & \multicolumn{1}{r}{\cellcolor[HTML]{E18500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{90DB00}{0.009}} & \multicolumn{1}{r}{\cellcolor[HTML]{E48100}{0.019}} & \multicolumn{1}{r}{\cellcolor[HTML]{EE6700}{0.014}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.022}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F55200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{ED6A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F06200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E08700}{0.035}} & \multicolumn{1}{r}{\cellcolor[HTML]{F15F00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{BEB700}{0.049}} & \multicolumn{1}{r}{\cellcolor[HTML]{E57E00}{0.027}} & \multicolumn{1}{r}{\cellcolor[HTML]{E87700}{0.048}} & \multicolumn{1}{r}{\cellcolor[HTML]{DF8A00}{0.022}} & \multicolumn{1}{r}{\cellcolor[HTML]{F55200}{0.010}} & \multicolumn{1}{r}{\cellcolor[HTML]{E57E00}{0.059}} & \multicolumn{1}{r}{\cellcolor[HTML]{E28300}{0.063}}\\
$\mid \Delta P_{t-5} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{ED6A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{B1C400}{0.033}} & \multicolumn{1}{r}{\cellcolor[HTML]{CEA400}{0.013}} & \multicolumn{1}{r}{\cellcolor[HTML]{C0B500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E48100}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E77A00}{0.057}} & \multicolumn{1}{r}{\cellcolor[HTML]{C1B300}{0.022}} & \multicolumn{1}{r}{\cellcolor[HTML]{BEB700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{ED6A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F45500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.052}} & \multicolumn{1}{r}{\cellcolor[HTML]{DC8E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F55200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{DF8A00}{0.012}} & \multicolumn{1}{r}{\cellcolor[HTML]{F45500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{ED6A00}{0.013}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.030}} & \multicolumn{1}{r}{\cellcolor[HTML]{F25C00}{0.050}} & \multicolumn{1}{r}{\cellcolor[HTML]{EA7200}{0.039}} & \multicolumn{1}{r}{\cellcolor[HTML]{DC8E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{ADC700}{0.073}}\\
$\mid \Delta P_{t-6} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{D79600}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74600}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E87700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{A7CC00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E77A00}{0.043}} & \multicolumn{1}{r}{\cellcolor[HTML]{D39C00}{0.010}} & \multicolumn{1}{r}{\cellcolor[HTML]{C5B000}{0.010}} & \multicolumn{1}{r}{\cellcolor[HTML]{F55200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E87700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{ED6A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EF6500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F15F00}{0.024}} & \multicolumn{1}{r}{\cellcolor[HTML]{EF6500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{DF8A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{D99400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EB7000}{0.029}} & \multicolumn{1}{r}{\cellcolor[HTML]{F35800}{0.014}} & \multicolumn{1}{r}{\cellcolor[HTML]{E97500}{0.019}} & \multicolumn{1}{r}{\cellcolor[HTML]{DF8A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{B9BC00}{0.063}}\\
$\sum_{i=7}^{i=12} \mid \Delta P_{t-i} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{AFC500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C1B300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{D69800}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{B7BE00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C9AA00}{0.107}} & \multicolumn{1}{r}{\cellcolor[HTML]{A9CA00}{0.078}} & \multicolumn{1}{r}{\cellcolor[HTML]{B3C200}{0.037}} & \multicolumn{1}{r}{\cellcolor[HTML]{9DD300}{0.052}} & \multicolumn{1}{r}{\cellcolor[HTML]{A0D100}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{D99400}{0.040}} & \multicolumn{1}{r}{\cellcolor[HTML]{C8AC00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F25C00}{0.116}} & \multicolumn{1}{r}{\cellcolor[HTML]{F93E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E57E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E48100}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E48100}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E28300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{D1A000}{0.135}} & \multicolumn{1}{r}{\cellcolor[HTML]{C5B000}{0.106}} & \multicolumn{1}{r}{\cellcolor[HTML]{9BD500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{DB9000}{0.040}} & \multicolumn{1}{r}{\cellcolor[HTML]{DF8A00}{0.069}} & \multicolumn{1}{r}{\cellcolor[HTML]{B3C200}{0.069}} & \multicolumn{1}{r}{\cellcolor[HTML]{D99400}{0.000}}\\
$\Delta P_{t-1}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{-0.040}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EE6700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{-0.032}} & \multicolumn{1}{r}{\cellcolor[HTML]{F15F00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EC6D00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{-0.076}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74600}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EC6D00}{0.000}}\\
$\Delta P_{t-2}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74600}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F93E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.004}} & \multicolumn{1}{r}{\cellcolor[HTML]{EC6D00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{-0.020}} & \multicolumn{1}{r}{\cellcolor[HTML]{F25C00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E77A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}}\\
$\Delta P_{t-3}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F55200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F55200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F64E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F06200}{0.000}}\\
$MO_{1000}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{-0.047}} & \multicolumn{1}{r}{\cellcolor[HTML]{F93E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E57E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EC6D00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F25C00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EA7200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74600}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.018}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F45500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F35800}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F45500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F35800}{0.002}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.011}} & \multicolumn{1}{r}{\cellcolor[HTML]{E28300}{0.005}} & \multicolumn{1}{r}{\cellcolor[HTML]{EA7200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EA7200}{-0.009}} & \multicolumn{1}{r}{\cellcolor[HTML]{E48100}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F93E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{D59A00}{-0.027}}\\
$MO_{2000}$ & \multicolumn{1}{r}{\cellcolor[HTML]{F45500}{-0.017}} & \multicolumn{1}{r}{\cellcolor[HTML]{E77A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{D59A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C6AE00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E87700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EF6500}{-0.057}} & \multicolumn{1}{r}{\cellcolor[HTML]{E97500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E48100}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{DF8A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EE6700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EC6D00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F64E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E48100}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E77A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EB7000}{-0.034}} & \multicolumn{1}{r}{\cellcolor[HTML]{E18500}{-0.017}} & \multicolumn{1}{r}{\cellcolor[HTML]{D29E00}{0.016}} & \multicolumn{1}{r}{\cellcolor[HTML]{F06200}{-0.062}} & \multicolumn{1}{r}{\cellcolor[HTML]{DE8C00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{D29E00}{-0.058}} & \multicolumn{1}{r}{\cellcolor[HTML]{DF8A00}{-0.041}} & \multicolumn{1}{r}{\cellcolor[HTML]{DF8A00}{-0.030}} & \multicolumn{1}{r}{\cellcolor[HTML]{D1A000}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F25C00}{0.000}}\\
$MO_{4000}$ & \multicolumn{1}{r}{\cellcolor[HTML]{93DA00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{90DB00}{-0.040}} & \multicolumn{1}{r}{\cellcolor[HTML]{A7CC00}{-0.050}} & \multicolumn{1}{r}{\cellcolor[HTML]{A4CE00}{-0.065}} & \multicolumn{1}{r}{\cellcolor[HTML]{73EA00}{-0.069}} & \multicolumn{1}{r}{\cellcolor[HTML]{88E000}{-0.020}} & \multicolumn{1}{r}{\cellcolor[HTML]{C5B000}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{A7CC00}{-0.042}} & \multicolumn{1}{r}{\cellcolor[HTML]{B5C000}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C6AE00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{7AE700}{-0.103}} & \multicolumn{1}{r}{\cellcolor[HTML]{B3C200}{-0.106}} & \multicolumn{1}{r}{\cellcolor[HTML]{BABB00}{-0.063}} & \multicolumn{1}{r}{\cellcolor[HTML]{B7BE00}{-0.068}} & \multicolumn{1}{r}{\cellcolor[HTML]{A0D100}{-0.013}} & \multicolumn{1}{r}{\cellcolor[HTML]{8EDD00}{-0.138}} & \multicolumn{1}{r}{\cellcolor[HTML]{AFC500}{-0.096}} & \multicolumn{1}{r}{\cellcolor[HTML]{B5C000}{-0.053}} & \multicolumn{1}{r}{\cellcolor[HTML]{CCA600}{-0.092}} & \multicolumn{1}{r}{\cellcolor[HTML]{BCB900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{BABB00}{-0.036}} & \multicolumn{1}{r}{\cellcolor[HTML]{A9CA00}{-0.037}} & \multicolumn{1}{r}{\cellcolor[HTML]{BEB700}{-0.021}} & \multicolumn{1}{r}{\cellcolor[HTML]{E87700}{0.000}}\\
$L_{DA}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.006}} & \multicolumn{1}{r}{\cellcolor[HTML]{F15F00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E97500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F93E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F45500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F25C00}{0.010}} & \multicolumn{1}{r}{\cellcolor[HTML]{EF6500}{0.043}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74600}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F55200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F06200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F45500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E67C00}{0.000}}\\
$O_{DA}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F64E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74600}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74600}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F93E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F55200}{-0.031}} & \multicolumn{1}{r}{\cellcolor[HTML]{EE6700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74600}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74600}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F64E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F93E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F06200}{-0.027}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{-0.003}} & \multicolumn{1}{r}{\cellcolor[HTML]{F55200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{DE8C00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{D79600}{0.000}}\\
$\Delta O$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{ED6A00}{0.000}}\\
$\Delta O_{planned}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F93E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F45500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F55200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E87700}{0.000}}\\
$\Delta O_{unplanned}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{ED6A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F93E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74600}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74600}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E87700}{0.000}}\\
$\mid P_{Spot} - P_{t-1} \mid$ & \multicolumn{1}{r}{\cellcolor[HTML]{E67C00}{0.047}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F55200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E57E00}{0.011}} & \multicolumn{1}{r}{\cellcolor[HTML]{E67C00}{0.071}} & \multicolumn{1}{r}{\cellcolor[HTML]{BCB900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F25C00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.068}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F35800}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F64E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{ED6A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.012}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F45500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E87700}{0.011}} & \multicolumn{1}{r}{\cellcolor[HTML]{F55200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}}\\
$SIDC$ & \multicolumn{1}{r}{\cellcolor[HTML]{DC8E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{ED6A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EF6500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F64E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EF6500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F25C00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F25C00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F06200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E67C00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F55200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EE6700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F64E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C9AA00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{D29E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F06200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E77A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E67C00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E77A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EF6500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F55200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EF6500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EC6D00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F06200}{0.000}}\\
$S_{DA}$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F64E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74600}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F45500}{-0.072}} & \multicolumn{1}{r}{\cellcolor[HTML]{E87700}{-0.077}} & \multicolumn{1}{r}{\cellcolor[HTML]{DA9200}{-0.085}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F45500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EF6500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E87700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F15F00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\Delta S^-$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F55200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F64E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E67C00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\Delta S^+$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F35800}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EB7000}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
$\sigma S$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F25C00}{0.052}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74600}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F93E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F06200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E18500}{0.019}} & \multicolumn{1}{r}{\cellcolor[HTML]{CCA600}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{ED6A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{-0.005}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}}\\
TTD & \multicolumn{1}{r}{\cellcolor[HTML]{84E200}{0.095}} & \multicolumn{1}{r}{\cellcolor[HTML]{56F400}{0.120}} & \multicolumn{1}{r}{\cellcolor[HTML]{C1B300}{0.153}} & \multicolumn{1}{r}{\cellcolor[HTML]{88E000}{0.141}} & \multicolumn{1}{r}{\cellcolor[HTML]{98D600}{0.180}} & \multicolumn{1}{r}{\cellcolor[HTML]{88E000}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C0B500}{0.061}} & \multicolumn{1}{r}{\cellcolor[HTML]{9BD500}{0.067}} & \multicolumn{1}{r}{\cellcolor[HTML]{A9CA00}{0.050}} & \multicolumn{1}{r}{\cellcolor[HTML]{D79600}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{A9CA00}{0.043}} & \multicolumn{1}{r}{\cellcolor[HTML]{E87700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EC6D00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{D39C00}{0.132}} & \multicolumn{1}{r}{\cellcolor[HTML]{BEB700}{0.078}} & \multicolumn{1}{r}{\cellcolor[HTML]{C6AE00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{A9CA00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{BCB900}{0.073}} & \multicolumn{1}{r}{\cellcolor[HTML]{B5C000}{0.049}} & \multicolumn{1}{r}{\cellcolor[HTML]{BABB00}{0.115}} & \multicolumn{1}{r}{\cellcolor[HTML]{8BDF00}{0.042}} & \multicolumn{1}{r}{\cellcolor[HTML]{96D800}{0.017}} & \multicolumn{1}{r}{\cellcolor[HTML]{A2D000}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{BABB00}{0.000}}\\
MON(d) & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F15F00}{0.050}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E08700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F45500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E48100}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{DC8E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{9DD300}{-0.029}} & \multicolumn{1}{r}{\cellcolor[HTML]{C5B000}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C5B000}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C6AE00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EA7200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F64E00}{-0.023}} & \multicolumn{1}{r}{\cellcolor[HTML]{DF8A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EC6D00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F93E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}}\\
SAT(d) & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{-0.018}} & \multicolumn{1}{r}{\cellcolor[HTML]{E67C00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F55200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E87700}{-0.021}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E97500}{0.025}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C0B500}{0.041}} & \multicolumn{1}{r}{\cellcolor[HTML]{DF8A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{B3C200}{0.041}} & \multicolumn{1}{r}{\cellcolor[HTML]{F64E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EC6D00}{0.023}} & \multicolumn{1}{r}{\cellcolor[HTML]{F06200}{0.030}} & \multicolumn{1}{r}{\cellcolor[HTML]{DE8C00}{0.005}} & \multicolumn{1}{r}{\cellcolor[HTML]{EF6500}{0.010}} & \multicolumn{1}{r}{\cellcolor[HTML]{F93E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F64E00}{0.000}}\\
SUN(d) & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F25C00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F06200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F64E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E48100}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EF6500}{0.047}} & \multicolumn{1}{r}{\cellcolor[HTML]{E67C00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C1B300}{0.012}} & \multicolumn{1}{r}{\cellcolor[HTML]{C6AE00}{0.046}} & \multicolumn{1}{r}{\cellcolor[HTML]{90DB00}{0.028}} & \multicolumn{1}{r}{\cellcolor[HTML]{D69800}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{D39C00}{0.011}} & \multicolumn{1}{r}{\cellcolor[HTML]{D1A000}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EC6D00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{DA9200}{0.006}} & \multicolumn{1}{r}{\cellcolor[HTML]{F06200}{0.000}}\\
$W_{DA}$ & \multicolumn{1}{r}{\cellcolor[HTML]{CFA200}{0.035}} & \multicolumn{1}{r}{\cellcolor[HTML]{C5B000}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{E87700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EC6D00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F15F00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{CBA800}{0.048}} & \multicolumn{1}{r}{\cellcolor[HTML]{ED6A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{D59A00}{0.015}} & \multicolumn{1}{r}{\cellcolor[HTML]{C6AE00}{0.048}} & \multicolumn{1}{r}{\cellcolor[HTML]{D59A00}{0.063}} & \multicolumn{1}{r}{\cellcolor[HTML]{DE8C00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{DC8E00}{0.049}} & \multicolumn{1}{r}{\cellcolor[HTML]{CFA200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{C3B200}{0.101}} & \multicolumn{1}{r}{\cellcolor[HTML]{AFC500}{0.091}} & \multicolumn{1}{r}{\cellcolor[HTML]{A9CA00}{0.053}} & \multicolumn{1}{r}{\cellcolor[HTML]{DB9000}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{B9BC00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{DB9000}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{A7CC00}{0.050}} & \multicolumn{1}{r}{\cellcolor[HTML]{C6AE00}{0.007}} & \multicolumn{1}{r}{\cellcolor[HTML]{E67C00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{B5C000}{0.059}} & \multicolumn{1}{r}{\cellcolor[HTML]{93DA00}{0.000}}\\
$\Delta W^-$ & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F25C00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74600}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F84200}{0.000}}\\
$\Delta W^+$ & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F93E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FA3900}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F35800}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.020}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F55200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F06200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FC2E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{DC8E00}{0.000}}\\
$\sigma W$ & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F45500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F15F00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F15F00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F74A00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FB3400}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F35800}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F55200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD2700}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F35800}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F64E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F55200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F93E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FD1E00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{FE1300}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F45500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{CFA200}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{F15F00}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{EF6500}{0.000}} & \multicolumn{1}{r}{\cellcolor[HTML]{DE8C00}{0.000}}\\
\bottomrule
\end{tabular}


==> TeX - Paper Submission Arxiv 1/tab_error_statistics.tex <==
\begin{tabular}{lrrrrrrrrrr}
\toprule
\multicolumn{1}{c}{ } & \multicolumn{4}{c}{Aggregate Statistics} & \multicolumn{3}{c}{Coverage Ratio} & \multicolumn{3}{c}{Winkler Score} \\
\cmidrule(l{3pt}r{3pt}){2-5} \cmidrule(l{3pt}r{3pt}){6-8} \cmidrule(l{3pt}r{3pt}){9-11}
 & MAE & RMSE & CRPS & ES & $	\text{CR}_{0.5}$ & $	\text{CR}_{0.9}$ & $	\text{CR}_{0.99}$ & $	\text{WS}_{0.5}$ & $	\text{WS}_{0.9}$ & $	\text{WS}_{0.99}$\\ 
 \midrule
Naive & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} \underline{\bfseries 3.178} & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} \underline{\bfseries 6.564} & {\cellcolor[HTML]{D5E21A}} \color[HTML]{000000} 1.222 & {\cellcolor[HTML]{8ED645}} \color[HTML]{000000} 17.271 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} \underline{\bfseries 0.491} & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} \underline{\bfseries 0.892} & {\cellcolor[HTML]{E7E419}} \color[HTML]{000000} 0.984 & {\cellcolor[HTML]{29AF7F}} \color[HTML]{F1F1F1} 8.676 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 12.922 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 36.218 \\
Auto.ARIMA & {\cellcolor[HTML]{39558C}} \color[HTML]{F1F1F1} 3.295 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 7.240 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 1.313 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 18.623 & {\cellcolor[HTML]{56C667}} \color[HTML]{000000} 0.407 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 0.713 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 0.845 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 9.544 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} \underline{\bfseries 9.269} & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} \underline{\bfseries 13.656} \\
MV.N & {\cellcolor[HTML]{C0DF25}} \color[HTML]{000000} 3.193 & {\cellcolor[HTML]{F4E61E}} \color[HTML]{000000} 6.570 & {\cellcolor[HTML]{48186A}} \color[HTML]{F1F1F1} 1.275 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 18.009 & {\cellcolor[HTML]{25858E}} \color[HTML]{F1F1F1} 0.680 & {\cellcolor[HTML]{B5DE2B}} \color[HTML]{000000} 0.927 & {\cellcolor[HTML]{B0DD2F}} \color[HTML]{000000} 0.972 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 9.364 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 16.392 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 25.500 \\
MV.t & {\cellcolor[HTML]{CAE11F}} \color[HTML]{000000} 3.191 & {\cellcolor[HTML]{F4E61E}} \color[HTML]{000000} 6.570 & {\cellcolor[HTML]{2CB17E}} \color[HTML]{F1F1F1} 1.240 & {\cellcolor[HTML]{1FA188}} \color[HTML]{F1F1F1} 17.495 & {\cellcolor[HTML]{2DB27D}} \color[HTML]{F1F1F1} 0.622 & {\cellcolor[HTML]{AADC32}} \color[HTML]{000000} 0.930 & {\cellcolor[HTML]{EFE51C}} \color[HTML]{000000} 0.986 & {\cellcolor[HTML]{31678E}} \color[HTML]{F1F1F1} 8.805 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 15.972 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 33.279 \\
RW.N & {\cellcolor[HTML]{7FD34E}} \color[HTML]{000000} 3.209 & {\cellcolor[HTML]{E5E419}} \color[HTML]{000000} 6.577 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 1.472 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 20.030 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 0.824 & {\cellcolor[HTML]{2FB47C}} \color[HTML]{F1F1F1} 0.970 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} \underline{\bfseries 0.989} & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 12.098 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 25.726 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 39.947 \\
RW.t & {\cellcolor[HTML]{B8DE29}} \color[HTML]{000000} 3.195 & {\cellcolor[HTML]{28AE80}} \color[HTML]{F1F1F1} 6.686 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 1.323 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 18.393 & {\cellcolor[HTML]{3C508B}} \color[HTML]{F1F1F1} 0.748 & {\cellcolor[HTML]{34B679}} \color[HTML]{F1F1F1} 0.968 & {\cellcolor[HTML]{E7E419}} \color[HTML]{000000} 0.996 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 9.888 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 23.068 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 63.616 \\
RW.t.Mix.D & {\cellcolor[HTML]{C5E021}} \color[HTML]{000000} 3.192 & {\cellcolor[HTML]{95D840}} \color[HTML]{000000} 6.616 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 1.304 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 18.171 & {\cellcolor[HTML]{33628D}} \color[HTML]{F1F1F1} 0.726 & {\cellcolor[HTML]{3BBB75}} \color[HTML]{F1F1F1} 0.964 & {\cellcolor[HTML]{E7E419}} \color[HTML]{000000} 0.996 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 9.624 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 21.941 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 61.102 \\
Mix.JSU & {\cellcolor[HTML]{EFE51C}} \color[HTML]{000000} 3.182 & {\cellcolor[HTML]{F1E51D}} \color[HTML]{000000} 6.571 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} \underline{\bfseries 1.218} & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} \underline{\bfseries 17.127} & {\cellcolor[HTML]{27AD81}} \color[HTML]{F1F1F1} 0.628 & {\cellcolor[HTML]{6ECE58}} \color[HTML]{000000} 0.947 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 0.991 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} \underline{\bfseries 8.519} & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 16.763 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 31.549 \\
Mix.SST & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 4.509 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 109.661 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 1.748 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 28.247 & {\cellcolor[HTML]{42BE71}} \color[HTML]{F1F1F1} 0.604 & {\cellcolor[HTML]{93D741}} \color[HTML]{000000} 0.936 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 0.989 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 12.427 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 17.356 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 33.674 \\
\bottomrule
\end{tabular}


==> TeX - Paper Submission Arxiv 1/tab_stationarity_tests.tex <==
\begin{tabular}{lllrrrrr}
\toprule
          							& Year 				&   2016 &   2017 &   2018 &   2019 &   2020 \\
Variable 							& Significance 		&        &        &        &        &        \\
\midrule
$\Delta P_{\text{ID},t}^{d,s}$ 		& $\alpha = 0.01$ &  0.675 &  0.658 &  0.633 &  0.596 &  0.555 \\
    	      						& $\alpha = 0.05$ &  0.750 &  0.744 &  0.717 &  0.684 &  0.641 \\
$P_{\text{ID},t}^{d,s}$ 			& $\alpha = 0.01$ &  0.059 &  0.055 &  0.055 &  0.059 &  0.088 \\
    	     						& $\alpha = 0.05$ &  0.128 &  0.125 &  0.122 &  0.117 &  0.157 \\
\bottomrule
\end{tabular}

==> TeX - Paper Submission Arxiv 1/tab_summary_statistics_delta_p.tex <==
\begin{tabular}{llrrrrr}
\toprule
                              &     &       2016 &       2017 &       2018 &       2019 &       2020 \\
\midrule
$\alpha_t$ 					  	& Count ($n$) 		&  257424 &  252960 &  268584 &  267096 &  158472 \\
                              	& Mean ($\mu$) &       0.82 &       0.87 &       0.95 &       0.98 &       0.98 \\
                              	& Std. ($\sigma$) &       0.39 &       0.34 &       0.23 &       0.14 &       0.15 \\ \midrule
$\Delta P_t \mid \alpha_t = 1$ 	& Count ($n$) &  209995 &  219258 &  253931 &  261721 &  154597 \\
                              	& Mean ($\mu$) &       0.02 &       0.02 &      -0.00 &      -0.00 &      -0.01 \\
                              	& Std. ($\sigma$) &       1.57 &       2.06 &       1.94 &       2.15 &       8.13 \\
		                        & MAD   			& 0.94 &       1.11 &       1.03 &       0.91 &       1.10 \\
								& IQR   			& 1.17 &       1.33 &       1.23 &       1.01 &       1.07 \\
								& Skewness     &       1.07 &       1.94 &       8.02 &      12.25 &       0.65 \\
								& Kurtosis &     131.50 &     322.14 &     902.99 &    2544.57 &   64968.44 \\
                              	& Min 				& -76.38 &    -127.70 &    -108.22 &    -214.16 &   -2161.80 \\
                              	& $Q_{0.10}$ &      -1.40 &      -1.61 &      -1.52 &      -1.29 &      -1.45 \\
                               & $Q_{0.25}$ &      -0.57 &      -0.65 &      -0.62 &      -0.51 &      -0.54 \\
                               & $Q_{0.50}$ &       0.00 &       0.00 &       0.00 &      -0.01 &       0.00 \\
                               & $Q_{0.75}$ &       0.60 &       0.68 &       0.61 &       0.50 &       0.53 \\
                               & $Q_{0.90}$ &       1.43 &       1.64 &       1.49 &       1.26 &       1.40 \\
                              & Max &      82.16 &     119.88 &     183.94 &     226.26 &    2164.23 \\
\bottomrule
\end{tabular}


==> TeX - Paper Submission Arxiv 1/tab_summary_statistics_outages.tex <==
\begin{tabular}{lrrr}
\toprule
{} &    $O_\text{DA}$ &  $\Delta O_\text{DA, 0,  planned}$ &  $\Delta O_\text{DA, 0,  unplanned}$ \\
\midrule
Count ($n$)     &  38856	&          38856 &            38856 \\
Mean ($\mu$)    &    15506.99 &                573.24 &                  410.07 \\
Std. ($\sigma$) &     5498.09 &                711.15 &                  486.55 \\
Min             &     5157.40 &              -3451.60 &                -1690.00 \\
$Q_{0.25}$      &    10585.90 &                 87.00 &                   49.30 \\
$Q_{0.50}$      &    15642.70 &                440.00 &                  271.05 \\
$Q_{0.75}$      &    19721.50 &                939.05 &                  634.00 \\
Max             &    33384.40 &               5569.00 &                 3847.00 \\
\bottomrule
\end{tabular}

==> TeX - Paper Submission Arxiv 1/tab_summary_statistics_wind_solar_demand.tex <==
\begin{tabular}{lrrrrrrr}
\toprule
{} & \multicolumn{3}{c@{}}{Wind} & \multicolumn{3}{c@{}}{Solar} &  \multicolumn{1}{c@{}}{Demand} \\ \cmidrule(lr){2-4} \cmidrule(l){5-7} \cmidrule(l){8-8}
{} & $\hat{W}$ & $\Delta \hat{W}$ & $\sigma(\Delta \hat{W})$ & $\hat{S}$ & $\Delta \hat{S}$ & $\sigma(\Delta \hat{S})$ & $\hat{D}$ \\
\midrule
Count ($n$)     &  38856 &         38856 &                 38856 &  38856 &         38856 &                 38856 &  38856 \\
Mean ($\mu$)    &  12372.39 &           -59.60 &                   182.78 &   4634.27 &             8.35 &                    56.22 &  59422.74 \\
Std. ($\sigma$) &   9410.80 &          1291.23 &                   110.11 &   6994.23 &           521.30 &                    84.29 &  10286.86 \\
Min             &    172.75 &         -9515.50 &                     6.00 &      0.00 &         -4604.50 &                     0.00 &  33927.90 \\
$Q_{0.25}$      &   5065.19 &          -680.56 &                   107.86 &      0.00 &            -2.25 &                     0.00 &  50884.18 \\
$Q_{0.50}$      &   9871.38 &           -44.25 &                   160.90 &    210.88 &             0.00 &                     3.79 &  59088.40 \\
$Q_{0.75}$      &  17295.94 &           546.06 &                   233.84 &   7497.25 &            14.00 &                    96.17 &  68029.13 \\
Max             &  47708.00 &         11383.25 &                  1940.55 &  32474.50 &          5914.50 &                   842.83 &  83494.50 \\
\bottomrule
\end{tabular}

==> TeX - Paper Submission Arxiv 1/tab_summary_statistics_wind_solar_demand_outages.tex <==
\begin{tabular}{lrrrrrrrrrr}
\toprule
{} &  \multicolumn{3}{c@{}}{Wind} & \multicolumn{3}{c@{}}{Solar} &    Demand & \multicolumn{3}{c@{}}{Outages} \\ \cmidrule(lr){2-4} \cmidrule(l){5-7} \cmidrule(l){8-8} \cmidrule(l){9-11} 
{} & $\hat{W}$ & $\Delta \hat{W}$ & $\sigma(\Delta \hat{W})$ & $\hat{S}$ & $\Delta \hat{S}$ & $\sigma(\Delta \hat{S})$ & $\hat{D}$ &       $O$ & $\Delta O_\text{planned}$ & $\Delta O_\text{unplanned}$ \\
\midrule
Count ($n$)     &  38856 &         38856 &                 38856 &  38856 &         38856 &                 38856 &  38856 &  38856 &            38856 &              38856 \\
Mean ($\mu$)    &  12372.39 &           -59.60 &                   182.78 &   4634.27 &             8.35 &                    56.22 &  59422.74 &  15506.99 &              573.24 &                410.07 \\
Std. ($\sigma$) &   9410.80 &          1291.23 &                   110.11 &   6994.23 &           521.30 &                    84.29 &  10286.86 &   5498.09 &              711.15 &                486.55 \\
Min             &    172.75 &         -9515.50 &                     6.00 &      0.00 &         -4604.50 &                     0.00 &  33927.90 &   5157.40 &            -3451.60 &              -1690.00 \\
% $Q_{0.25}$      &   5065.19 &          -680.56 &                   107.86 &      0.00 &            -2.25 &                     0.00 &  50884.18 &  10585.90 &               87.00 &                 49.30 \\
% $Q_{0.50}$      &   9871.38 &           -44.25 &                   160.90 &    210.88 &             0.00 &                     3.79 &  59088.40 &  15642.70 &              440.00 &                271.05 \\
% $Q_{0.75}$      &  17295.94 &           546.06 &                   233.84 &   7497.25 &            14.00 &                    96.17 &  68029.13 &  19721.50 &              939.05 &                634.00 \\
Max             &  47708.00 &         11383.25 &                  1940.55 &  32474.50 &          5914.50 &                   842.83 &  83494.50 &  33384.40 &             5569.00 &               3847.00 \\
\bottomrule
\end{tabular}


==> tab_summary_statistics_outages.tex <==
\begin{tabular}{lrrr}
\toprule
{} &    $O_\text{DA}$ &  $\Delta O_\text{DA, 0,  planned}$ &  $\Delta O_\text{DA, 0,  unplanned}$ \\
\midrule
Count ($n$)     &  38856	&          38856 &            38856 \\
Mean ($\mu$)    &    15506.99 &                573.24 &                  410.07 \\
Std. ($\sigma$) &     5498.09 &                711.15 &                  486.55 \\
Min             &     5157.40 &              -3451.60 &                -1690.00 \\
$Q_{0.25}$      &    10585.90 &                 87.00 &                   49.30 \\
$Q_{0.50}$      &    15642.70 &                440.00 &                  271.05 \\
$Q_{0.75}$      &    19721.50 &                939.05 &                  634.00 \\
Max             &    33384.40 &               5569.00 &                 3847.00 \\
\bottomrule
\end{tabular}

==> tab_summary_statistics_wind_solar_demand.tex <==
\begin{tabular}{lrrrrrrr}
\toprule
{} & \multicolumn{3}{c@{}}{Wind} & \multicolumn{3}{c@{}}{Solar} &  \multicolumn{1}{c@{}}{Demand} \\ \cmidrule(lr){2-4} \cmidrule(l){5-7} \cmidrule(l){8-8}
{} & $\hat{W}$ & $\Delta \hat{W}$ & $\sigma(\Delta \hat{W})$ & $\hat{S}$ & $\Delta \hat{S}$ & $\sigma(\Delta \hat{S})$ & $\hat{D}$ \\
\midrule
Count ($n$)     &  38856 &         38856 &                 38856 &  38856 &         38856 &                 38856 &  38856 \\
Mean ($\mu$)    &  12372.39 &           -59.60 &                   182.78 &   4634.27 &             8.35 &                    56.22 &  59422.74 \\
Std. ($\sigma$) &   9410.80 &          1291.23 &                   110.11 &   6994.23 &           521.30 &                    84.29 &  10286.86 \\
Min             &    172.75 &         -9515.50 &                     6.00 &      0.00 &         -4604.50 &                     0.00 &  33927.90 \\
$Q_{0.25}$      &   5065.19 &          -680.56 &                   107.86 &      0.00 &            -2.25 &                     0.00 &  50884.18 \\
$Q_{0.50}$      &   9871.38 &           -44.25 &                   160.90 &    210.88 &             0.00 &                     3.79 &  59088.40 \\
$Q_{0.75}$      &  17295.94 &           546.06 &                   233.84 &   7497.25 &            14.00 &                    96.17 &  68029.13 \\
Max             &  47708.00 &         11383.25 &                  1940.55 &  32474.50 &          5914.50 &                   842.83 &  83494.50 \\
\bottomrule
\end{tabular}
